ChatPCG: Large Language Model-Driven Reward Design for Procedural Content Generation

Driven by the rapid growth of machine learning, recent advances in game artificial intelligence (AI) have significantly impacted productivity across various gaming genres. Reward design plays a pivotal role in training game AI models, wherein researchers implement concepts of specific reward functions. However, despite the presence of AI, the reward design process predominantly remains in the domain of human experts, as it is heavily reliant on their creativity and engineering skills. Therefore, this paper proposes ChatPCG, a large language model (LLM)-driven reward design framework.It leverages human-level insights, coupled with game expertise, to generate rewards tailored to specific game features automatically. Moreover, ChatPCG is integrated with deep reinforcement learning, demonstrating its potential for multiplayer game content generation tasks. The results suggest that the proposed LLM exhibits the capability to comprehend game mechanics and content generation tasks, enabling tailored content generation for a specified game. This study not only highlights the potential for improving accessibility in content generation but also aims to streamline the game AI development process.

==> discussion/discussion.tex <==
discussion!


==> experiment/Experiment1.tex <==
\subsection{Comparisons}

\begin{itemize}

\item \textbf{Winrate Reward} ($R_{WR}$) ensures the generated contents satisfied the designer-desired winrate result. The L1 norm distance to the goal, $l$, is calculated as $l_t=abs(||g_t-p_t||_{L1})$, where $p_t$ represents the playtested winrate at time $t$.
The reward at time $t$ is then calculated as $r_{t}=l_{t-1}-l_{t}$.

\item \textbf{LLM Reward} ($R_{LLM}$) is measured by the LLM-generated reward function.
The function computes the reward by taking as input the playtested results at time $t$.

\item \textbf{Hybrid Reward} ($R_{HYB}$) combines winrate and LLM-generated rewards with the weights for obtaining the winrate ($w_{WR}$) and LLM ($w_{LLM}$). The hybrid reward represented as $R_{HYB}=R_{WR}*w_{WR}+R_{LLM}*w_{LLM}$.

\end{itemize}

The winrate reward is the baseline proposed on a previous work \cite{jeon2023raidenv} and the LLM- and hybrid rewards are newly proposed in this paper to consider game characteristic on reward design.

\subsection{Experiment Setting}
The DRL models are trained 20K steps through three different reward functions in the comparisons; the detailed model settings follow previous work \cite{jeon2023raidenv} and results are reported with averaged value from three runs.
In generation of LLM-based reward, we employ OpenAI's \texttt{gpt-4-turbo} model as backend language model and repeated self-alignment process for $N_{revision}=5$ times.
The weights set to $w_{WR}=0.1$ and $w_{LLM}=0.3$ for hybrid reward function.
For evaluation, 1K character configurations are sampled from the trained DRL agents.

\subsection{Evaluation Metrics}
The generated contents are evaluate in three criteria: controllability, diversity, and team build score.
The details of controllability and diversity criteria are described on previous work \cite{jeon2023raidenv}.
Team build score is newly proposed in this work to consider the multiplayer game design \cite{rosen2011managing}, role differentiation.
The direction of the arrows indicates superior values.

\textbf{Controllability (Ctr, $\downarrow$)} measures mean of error values between the current ($W_c$) and the target ($W_t$) winrates.
The lower error indicates that the model successfully generated the designer-desired contents.
Ctr is measured with Eq. \ref{eq:Controllability}, where $N$ denotes the number of samples and $W_{i,c}$ denotes the current winrate of $i$th sample.

\begin{align}
\label{eq:Controllability}
\text{Ctr} = \frac{1}{N} \sum_{i=1}^{N} abs(||W_{t}-W_{i,c}||_{L1})
\end{align}

\textbf{Diversity (Div, $\uparrow$)} measures the variety of character candidates that satisfy the generation condition. 
The valid samples, the winrate error is lower than threshold (i.e., $abs(||W_{t}-W_{i,c}||_{L1}<0.1$), are selected on diversity measurement.
The dimension reduction technique \cite{wold1987principal} is applied to the generated character properties for reducing the dimension six to one.
Div calculates the standard deviation of the dimension-reduced values.

\textbf{Team Build Score (Tbs, $\uparrow$)} measures the degree of role differentiation for a team.
Tbs is measured with Eq. \ref{eq:tbs}, where $A$ denotes the agent sets in a team; $K$ denotes set of character properties.
$S(a_i,k)$ represent the normalized value of $i$th agent's $k$ property in a state $S$.
The mean of property values are calculate in pairwise among agents.
We assume that the higher mean of distances represents the distinct character roles in cooperative setting.
The mean Tbs value on the valid samples are reported in result.

\begin{align}
\label{eq:tbs}
\text{Tbs($A$)} = \frac{1}{\binom{|A|}{2}} \sum_{(a_i, a_j) \in A, i < j} \left( \frac{1}{K} \sum_{k \in K} \left| S(a_i,k) - S(a_j,k) \right| \right)
\end{align}

\subsection{Experimental Result}
\input{experiment/Result1.tex}

Table \ref{tab:evaluation} 
